Statistical modeling of quantum error propagation

In this paper, I design a new statistical abstract model for studying quantum error propagation. For each circuit, I give the algorithm to construct the Error propagation space-time graph(\textbf{EPSTG}) graph as well as the bipartite reverse spanning graph (\textbf{RSG}). Then I prove that the problem of finding an error pattern is $\mathcal{P}$ while calculate the error number distribution is $\textit{NP-complete}$. I invent the new measure for error propagation and show that for widely used transversal $CNOT$ circuit in parallel, the shift of distribution is bounded by $\frac{n}{27}$, where $n$ is the number of physical qubits. The consistency between the result of qiskit simulation and my algorithm justify the correctness of my model. Applying the framework to random circuit, I show that there is severe unbounded error propagation when circuit has global connection. We also apply my framework on parallel transversal logical $CNOT$ gate in surface code, and demonstrate that the error threshold will decrease from $0.231$ to $0.134$ per cycle.

==> conductance.tex <==



\section{Conductance of graph}

SS

==> counting.tex <==
\section{Exact algorithm by counting}






\subsection{Counting complexity}


Weighted Counting Constraint Satisfaction Problems $(\#CSPs)$


\subsection{A parsimononious reduction}

==> measure.tex <==
\section{Measure of distribution}


In this section, I propose the measure of how close are two distribution.



\subsection{Kullback–Leibler divergence}

Assume that we have two distributions $P$ and $Q$, which share the same sample space $\mathcal{X}$, the Kullback–Leibler(\textbf{KL}) divergence is defined as:

\begin{equation}
    D_{KL}(P||Q)=\sum_{x \in \mathcal{X}} P(x) \log(\frac{P(x)}{Q(x)})
    \label{eq:KLdivergence}
\end{equation}



{\color{red} We wish that we could get a formula such that \autoref{eq:KLdivergence} is related with the number of CNOT gates, the error probability, and the structure of the circuit.}






==> qiskit.tex <==
\section{Qiskit experiment}



